SCALES for Keck: Optical Design

SCALES is a high-contrast, infrared coronagraphic imager and integral field spectrograph (IFS) to be deployed behind the W.M. Keck Observatory adaptive optics system. A reflective optical design allows diffraction-limited imaging over a large wavelength range (1.0 - 5.0 microns). A microlens array-based IFS coupled with a lenslet reformatter ("slenslit") allow spectroscopy at both low (R = 35 - 250) and moderate (R = 2000 - 6500) spectral resolutions. The large wavelength range, diffraction-limited performance, high contrast coronagraphy and cryogenic operation present a unique optical design challenge. We present the full SCALES optical design, including performance modeling and analysis and manufacturing.

==> A-Doc_formatting_inputs/sc_0010_100_aliases_astro_phys_optic.tex <==
% !TEX encoding = UTF-8 Unicode
% -*- coding: UTF-8; -*-
% vim: set fenc=utf-8
%
% Astronomy, Physics, and Optics terms

%: Astronomy
\newcommand{\hband}{H-band}
\newcommand{\jband}{J-band}
\newcommand{\kband}{K-band}

%: Physics
\newcommand{\snratio}{\ensuremath{SNR}}

%: Optics
\newcommand{\aoifull}{Angle of Incidence}
\newcommand{\aoi}{AOI}
\newcommand{\eedfull}{Encircle Energy Diagram}
\newcommand{\eed}{EED}
\newcommand{\eflfull}{Effective Focal Length}
\newcommand{\eflab}{EFL}
\newcommand{\evec}{\ensuremath{E}}
\newcommand{\fovfull}{Field of View}
\newcommand{\fovab}{FOV}
\newcommand{\fwhm}{FWHM}
\newcommand{\fwhmfull}{Full Width at Half Maximum}
\newcommand{\hwpfull}{Half-wave Plate}
\newcommand{\hwp}{HWP}
\newcommand{\ifu}{IFU}
\newcommand{\ifufull}{Integral Field Unit}
\newcommand{\ovec}{\ensuremath{O}}
\newcommand{\qwpfull}{Quarter-wave Plate}
\newcommand{\qwp}{QWP}
\newcommand{\sun}{\odot}

%: Terms taking arguments
\newcommand{\fnum}[1]{\ensuremath{f/#1}}

% hg wants a blank line at EOF:


==> A-Doc_formatting_inputs/sc_0010_100_aliases_units.tex <==
% Aliases for non-SI units to use with the SIunits package.
% Aliases for formatting a range of numbers with with consistent spacing.
% Aliases for formatting a range of values with units.

%: Textual symbols
%:   number grouping
%    Memoir uses \fcardinal for numbers larger than 0.
%    If we used the siunitx package we could get nice spacing with \num{}
%    But we use SIunits.
%    Sytlistically, we should use a \thinspace = \, = 3/18 between number groups, but sometimes 2/18 em looks better:
\newcommand{\ngspace}{\;\!} % ng for number-space; (5-3)/18 = 2/18; \!=\negthinspace

%:   \simspace
\newcommand{\simspace}{\ensuremath{\sim\;\!}} % (5-3)/18 = 2/18

%:   \unitendash, for use with \unit
\newcommand{\unitendash}{\ensuremath{\!\text{--}}}

%: non-SI units
\newcommand{\adu}{ADU}
\newcommand{\arcdeg}{arcdeg}
\newcommand{\arcmin}{arcmin}
\newcommand{\arcminutetext}{arc minute} % \arcminute give prime symbol
\newcommand{\arcminutestext}{arcminutes}
\newcommand{\arcsectext}{arcsec}
\newcommand{\au}{AU}
\newcommand{\awg}{AWG}
\newcommand{\degab}{deg}
\newcommand{\degreetext}{degree}
\newcommand{\degreestext}{degrees}
\newcommand{\electron}{\ensuremath{e^{-}}}
\newcommand{\feet}{feet}
\newcommand{\foot}{foot}
\newcommand{\gauss}{G}
\newcommand{\hours}{hours}  % note \hour resolves to h
\newcommand{\inch}{inch}
\newcommand{\inchab}{in}
\newcommand{\kpc}{kpc}
\newcommand{\lines}{lines}
\newcommand{\magnitude}{mag}
\newcommand{\micron}{\micro\metre}
\newcommand{\microns}{\micro\metre}
\newcommand{\mjup}{\ensuremath{\textrm{M}_{Jup}}}
\newcommand{\mm}{\milli\metre}
\newcommand{\mrad}{\milli\rad}  % A cheat \rad in siunits pkg is for radiation - but results in correct textual abbrev for milliradians = mrad.
\newcommand{\parsec}{pc}
\newcommand{\perpixel}{\reciprocal\pixel}
\newcommand{\pixel}{pixel}
\newcommand{\pixels}{pixels}
\newcommand{\port}{port}
\newcommand{\poundab}{lb}
\newcommand{\poundmass}{lb\ensuremath{_m}}
\newcommand{\secondstext}{seconds}
\newcommand{\step}{step}
\newcommand{\steps}{steps}
\newcommand{\stepsperrev}{steps/rev}
\newcommand{\torr}{Torr}
\newcommand{\rackunit}{U}
\newcommand{\percent}{\!\%} % one neg space (-3/18em) w/ \units
\newcommand{\umonth}{month}
\newcommand{\umonths}{months}
\newcommand{\wattstext}{Watts}
\newcommand{\yearunit}{yr}
\newcommand{\years}{years}
\newcommand{\photons}{photons}

%added by RDS
\newcommand{\arcsecondstext}{arcseconds} %2021-10-06
\newcommand{\arcsecondtext}{arcsecond} %2021-10-06
\newcommand{\spaxel}{spaxel} %2021-10-06
\newcommand{\arcsec}{arcsec} %2021-10-06

%: Spacing a range of numbers
%\newcommand{\numrange}[2]{\ensuremath{#1\text{--}#2}} % defined in siunitx, not siunits
\newcommand{\numrange}[2]{\ensuremath{#1\,\,\unitendash\,#2}} % defined in siunitx, not siunits

%: Spacing for a range of units with an endash:
%:   Example spacing option 1 using new command \num and \unit
%:   N.B. \num defined in siunitx, not SIunits
\newcommand{\num}[1]{\ensuremath{#1}}
%%   \num{1.02}--\unit{1.79}{\micro\metre}
%%
%:   Example spacing option 2 using \unit and new command \unitendash
%%   \unit{1.02}{\unitendash}\unit{1.79}{\micron}
%%
%:   Example spacing option 3 using new command \urange and \unitendash
\newcommand{\urange}[3]{\ensuremath{#1\,\,\unitendash\,#2\:\text{#3}}}
%\newcommand{\urange}[3]{\ensuremath{#1\,\text{--}\,#2\:\text{#3}}}


\endinput

%% Put this in blank doc and uncomment to compare:
%1.02--1.79 \micron\@ = Endash plain\\
%\num{1.02}--\num{1.79}~\micron\@ = Endash nums\\
%\num{1.02}--\unit{1.79}{\micron} = Endash num to unit\\
%\unit{1.02}{\text{--}}\unit{1.79}{\micron} = unit and text endash\\
%\unit{1.02}{\!\text{--}}\unit{1.79}{\micron} = unit w neg space and text endash ** \\
%\unit{1.02}{\!-}\unit{1.79}{\micron} = Unit with neg space and minus(?)\\
%\unit{1.02}{\micron}--\unit{1.79}{\micron}

% hg wants a blank line at EOF:


==> A-Doc_formatting_inputs/sc_0010_101_pkginputs.tex <==
% !TEX encoding = UTF-8 Unicode
% -*- coding: UTF-8; -*-
% vim: set fenc=utf-8
%
%-=-=-=-=-=--=-=--=-=-=-=--=-=-=-=-=-=-=-=-=-
% REVISION HISTORY
%-=-=-=-=-=--=-=--=-=-=-=--=-=-=-=-=-=-=-=-=-
%% Packages required for SCALES documents
%% 2012-06-11  SNR
%% UF Astro latex packages are in /usr/share/texmf/tex/latex
%% Are fonts located elsewhere?
%-=-=-=-=-=--=-=--=-=-=-=--=-=-=-=-=-=-=-=-=-
%%  Recouped by RDS 2018 for SCALES

%-----------------------------------------------------------------
%% Fonts packages
%% Before this pkginputs file is loaded, the style file mi_mwd_003_03.sty inputs these fonts packages:
%% \usepackage[T1]{fontenc}
%% \usepackage[utf8]{inputenc}
%% \usepackage[sc,osf]{mathpazo}
%% \usepackage[scaled]{helvet}  % for ss fonts
%% \usepackage{courier}  % for tt fonts

%\usepackage{fixltx2e}%[2006/09/13]
\usepackage{algorithm}
\usepackage{algpseudocode}
\usepackage{alphalph}
\usepackage{amsmath}
\usepackage{amssymb}
%\usepackage{chapterbib} % compatible with memoir, need include?
\usepackage[yyyymmdd]{datetime}
\usepackage{etoolbox}
\usepackage{eurosym}
\usepackage[table,usenames,dvipsnames]{xcolor}
\usepackage{graphicx}
\DeclareGraphicsExtensions{.png,pdf}
\usepackage{lscape} % from Paco
\usepackage{longtable}
\usepackage{mathtools}
\usepackage[stretch=10]{microtype} % pdflatex only ; 1% font expansion
%\usepackage{natbib}
%Import the natbib package and sets a bibliography style
\usepackage[round,authoryear,semicolon]{natbib}
\bibliographystyle{C-End-Matter/apj.bst}
%\usepackage{biblatex}
\usepackage{aas_macros}
\usepackage{paralist}
\usepackage{ragged2e}
\usepackage{rotating}
\usepackage[binary,squaren,cdot,thickqspace,thickspace]{SIunits}  % cdot font problem? Seems like the thickqspace isn't working either :( -RDS 16 aug 2021
\usepackage{xfrac}
\usepackage[normalem]{ulem}
\usepackage{textcomp}
\usepackage{url}
\usepackage{wrapfig}
\usepackage{multirow}
\usepackage{xargs}                      % Use more than one optional parameter in a new commands, particularly useful for the \todo custom commands
\usepackage{hyperref}  % HYPERREF Must be last loaded package.

%: hg wants a blank line at EOF


==> A-Doc_formatting_inputs/sc_0010_104_aastex_aliases.tex <==
\newcommand\aj{AJ}%
          % Astronomical Journal
\newcommand\actaa{Acta Astron.}%
  % Acta Astronomica
\newcommand\araa{ARA\&A}%
          % Annual Review of Astron and Astrophys
\newcommand\apj{ApJ}%
          % Astrophysical Journal
\newcommand\apjl{ApJ}%
          % Astrophysical Journal, Letters
\newcommand\apjs{ApJS}%
          % Astrophysical Journal, Supplement
\newcommand\ao{Appl.~Opt.}%
          % Applied Optics
\newcommand\apss{Ap\&SS}%
          % Astrophysics and Space Science
\newcommand\aap{A\&A}%
          % Astronomy and Astrophysics
\newcommand\aapr{A\&A~Rev.}%
          % Astronomy and Astrophysics Reviews
\newcommand\aaps{A\&AS}%
          % Astronomy and Astrophysics, Supplement
\newcommand\azh{AZh}%
          % Astronomicheskii Zhurnal
\newcommand\baas{BAAS}%
          % Bulletin of the AAS
\newcommand\caa{Chinese Astron. Astrophys.}%
  % Chinese Astronomy and Astrophysics
\newcommand\cjaa{Chinese J. Astron. Astrophys.}%
  % Chinese Journal of Astronomy and Astrophysics
\newcommand\icarus{Icarus}%
  % Icarus
\newcommand\jcap{J. Cosmology Astropart. Phys.}%
  % Journal of Cosmology and Astroparticle Physics
\newcommand\jrasc{JRASC}%
          % Journal of the RAS of Canada
\newcommand\memras{MmRAS}%
          % Memoirs of the RAS
\newcommand\mnras{MNRAS}%
          % Monthly Notices of the RAS
\newcommand\na{New A}%
  % New Astronomy
\newcommand\nar{New A Rev.}%
  % New Astronomy Review
\newcommand\pra{Phys.~Rev.~A}%
          % Physical Review A: General Physics
\newcommand\prb{Phys.~Rev.~B}%
          % Physical Review B: Solid State
\newcommand\prc{Phys.~Rev.~C}%
          % Physical Review C
\newcommand\prd{Phys.~Rev.~D}%
          % Physical Review D
\newcommand\pre{Phys.~Rev.~E}%
          % Physical Review E
\newcommand\prl{Phys.~Rev.~Lett.}%
          % Physical Review Letters
\newcommand\pasa{PASA}%
  % Publications of the Astron. Soc. of Australia
\newcommand\pasp{PASP}%
          % Publications of the ASP
\newcommand\pasj{PASJ}%
          % Publications of the ASJ
\newcommand\qjras{QJRAS}%
          % Quarterly Journal of the RAS
\newcommand\rmxaa{Rev. Mexicana Astron. Astrofis.}%
  % Revista Mexicana de Astronomia y Astrofisica
\newcommand\skytel{S\&T}%
          % Sky and Telescope
\newcommand\solphys{Sol.~Phys.}%
          % Solar Physics
\newcommand\sovast{Soviet~Ast.}%
          % Soviet Astronomy
\newcommand\ssr{Space~Sci.~Rev.}%
          % Space Science Reviews
\newcommand\zap{ZAp}%
          % Zeitschrift fuer Astrophysik
\newcommand\nat{Nature}%
          % Nature
\newcommand\iaucirc{IAU~Circ.}%
          % IAU Cirulars
\newcommand\aplett{Astrophys.~Lett.}%
          % Astrophysics Letters and Communications
\newcommand\apspr{Astrophys.~Space~Phys.~Res.}%
          % Astrophysics Space Physics Research
\newcommand\bain{Bull.~Astron.~Inst.~Netherlands}%
          % Bulletin Astronomical Institute of the Netherlands
\newcommand\fcp{Fund.~Cosmic~Phys.}%
          % Fundamental Cosmic Physics
\newcommand\gca{Geochim.~Cosmochim.~Acta}%
          % Geochimica Cosmochimica Acta
\newcommand\grl{Geophys.~Res.~Lett.}%
          % Geophysics Research Letters
\newcommand\jcp{J.~Chem.~Phys.}%
          % Journal of Chemical Physics
\newcommand\jgr{J.~Geophys.~Res.}%
          % Journal of Geophysical Research
\newcommand\jqsrt{J.~Quant.~Spec.~Radiat.~Transf.}%
          % Journal of Quantitiative Spectroscopy and Radiative Trasfer
\newcommand\memsai{Mem.~Soc.~Astron.~Italiana}%
          % Mem. Societa Astronomica Italiana
\newcommand\nphysa{Nucl.~Phys.~A}%
          % Nuclear Physics A
\newcommand\physrep{Phys.~Rep.}%
          % Physics Reports
\newcommand\physscr{Phys.~Scr}%
          % Physica Scripta
\newcommand\planss{Planet.~Space~Sci.}%
          % Planetary Space Science
\newcommand\procspie{Proc.~SPIE}%
          % Proceedings of the SPIE

==> Tables/DisperserSpecs.tex <==
% !TEX encoding = UTF-8 Unicode
% -*- coding: UTF-8; -*-
% vim: set fenc=utf-8

\begin{tabular}{c | c }
\textbf{Wavelength range [\num{}{\micro\meter}]} & \textbf{Mid-band spectral resolution}   \\
\midrule
\numrange{1.95}{2.45} (K-band) & R = $150$     \\
\numrange{4.5}{5.2} (M-band) & R = $70$     \\
\numrange{2.9}{4.15} (L-band) & R = $40$      \\
\numrange{2.0}{5.0} (SEDS) & R = $10$    \\
\numrange{3.1}{3.5} (CH\textsubscript{4}+PAH)   \\
\numrange{2.0}{4.0} (water ice) & R = $30$    \\
\numrange{1.95}{2.45} (K-band) & R = \\
\numrange{2.9}{4.15}  (L-band) & R = \\
\numrange{4.5}{5.2}  (M-band) & R = \\
\bottomrule
\end{tabular}
